An Explainable Adversarial Robustness Metric for Deep Learning Neural Networks

Deep Neural Networks(DNN) have excessively advanced the field of computer vision by achieving state of the art performance in various vision tasks. These results are not limited to the field of vision but can also be seen in speech recognition and machine translation tasks. Recently, DNNs are found to poorly fail when tested with samples that are crafted by making imperceptible changes to the original input images. This causes a gap between the validation and adversarial performance of a DNN. An effective and generalizable robustness metric for evaluating the performance of DNN on these adversarial inputs is still missing from the literature. In this paper, we propose Noise Sensitivity Score (NSS), a metric that quantifies the performance of a DNN on a specific input under different forms of fix-directional attacks. An insightful mathematical explanation is provided for deeply understanding the proposed metric. By leveraging the NSS, we also proposed a skewness based dataset robustness metric for evaluating a DNN's adversarial performance on a given dataset. Extensive experiments using widely used state of the art architectures along with popular classification datasets, such as MNIST, CIFAR-10, CIFAR-100, and ImageNet, are used to validate the effectiveness and generalization of our proposed metrics. Instead of simply measuring a DNN's adversarial robustness in the input domain, as previous works, the proposed NSS is built on top of insightful mathematical understanding of the adversarial attack and gives a more explicit explanation of the robustness.

==> backup_old_content.tex <==
% \begin{table*}[ht]
% \caption{DenseNet architectures for CIFAR datasets. The growth rate for all the networks is $k=12$. Each "conv" is a composite unit comprising the sequence of BN-RELU-Convolution layer.}

% \centering
% \scalebox{0.8}{
% \begin{tabular}
% {c|c|c|c|c|c}
% \hline
%   & & & & &\\
% Layers & Output Size & DenseNet-40 & DenseNet-40-H1 & DenseNet-40-H2 & DenseNet-40-H3\\[0.5ex]
% \hline
% \makecell{Pre-Activation\\Convolution} & $32\times32$ & \multicolumn{4}{c}{$3\times3$ convolution layer} \\ [0.5ex]
% \hline

% & & & & &\\
% \multirow{3}{*}{Dense Block (1)} & \multirow{3}{*}{$32\times32$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv} \\
%        \textrm{12 kernels}
%      \end{bmatrix}\times 12$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv}\\
%        12*(n+2) \textrm{ kernels}\\
%        n=0,...,11  
%      \end{bmatrix}\times 12$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv} \\
%        \textrm{12 kernels}
%      \end{bmatrix}\times 12$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv} \\
%        \textrm{12 kernels}
%      \end{bmatrix}\times 12$}\\[0.5ex] 
%   & & & & &\\[0.5ex]
%   & & & & &\\[0.5ex]
% \hline

% \makecell{Transition Layer\\(1)} & $16\times16$ & \multicolumn{4}{c}{$1\times1$ conv, $2\times2$ average pool, stride 2}\\ [0.5ex]
% \hline

% & & & & &\\
% \multirow{3}{*}{Dense Block (2)} & \multirow{3}{*}{$16\times16$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv} \\
%        \textrm{12 kernels}
%      \end{bmatrix}\times 12$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv}\\
%        12 \textrm{ kernels}
%      \end{bmatrix}\times 12$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv} \\
%        12*(n+2) \textrm{ kernels} \\
%        n=13,...,24  
%      \end{bmatrix}\times 12$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv} \\
%        \textrm{12 kernels}
%      \end{bmatrix}\times 12$}\\[0.5ex]  
%   & & & & &\\[0.5ex]
%   & & & & &\\[0.5ex]
% \hline

% \makecell{Transition Layer\\(2)} & $8\times8$ & \multicolumn{4}{c}{$1\times1$ conv, $2\times2$ average pool, stride 2} \\ [0.5ex]
% \hline

% & & & & &\\
% \multirow{3}{*}{Dense Block (3)} & \multirow{3}{*}{$8\times8$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv} \\
%        \textrm{12 kernels}
%      \end{bmatrix}\times 12$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv}\\
%        12 \textrm{ kernels}
%      \end{bmatrix}\times 12$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv} \\
%        12 \textrm{ kernels}
%      \end{bmatrix}\times 12$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv} \\
%        12*(n+2) \textrm{ kernels} \\
%        n=25,...,36  
%      \end{bmatrix}\times 12$}\\[0.5ex] 
%   & & & & &\\[0.5ex]
%   & & & & &\\[0.5ex]
% \hline

% \makecell{Classification\\ Layer} & $1\times1$ & \multicolumn{4}{c}{$8\times8$ global average pool, 10D fully-connected, Softmax} \\ [0.5ex]
% \hline

% \end{tabular}}
% \label{table1}
% \end{table*}

% \begin{table*}[ht]
% \caption{ResNet architectures for CIFAR datasets.}

% \centering
% \scalebox{0.7}{
%  \begin{tabular}{c|c|c|c|c|c}
% \hline
%   & & & & &\\
% Layers & Output Size & ResNet-18 & ResNet-18-H2 & ResNet-18-H3 & ResNet-18-H4\\[0.5ex]
% \hline
% \makecell{Pre-Activation\\Convolution} & $32\times32$ & \multicolumn{4}{c}{$3\times3$ convolution layer, BN, ReLU} \\ [0.5ex]
% \hline
% Block (1) & $32\times32$ & \multicolumn{4}{c}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN}
%      \end{bmatrix}\times 2$} \\[0.5ex] 
% \hline
%   & & & & &\\[0.5ex]
% \multirow{3}{*}{Block (2)} & \multirow{3}{*}{$16\times16$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN} \\
%        1\times1 \textrm{ conv, stride 2}
%      \end{bmatrix}\times 2$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN}
%      \end{bmatrix}\times 2$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN} \\
%        1\times1 \textrm{ conv, stride 2}
%      \end{bmatrix}\times 2$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN} \\
%        1\times1 \textrm{ conv, stride 2}
%      \end{bmatrix}\times 2$} \\[0.5ex] 
%   & & & & &\\[0.5ex]
%   & & & & &\\[0.5ex]
% \hline
%   & & & & &\\[0.5ex]
% \multirow{3}{*}{Block (3)} & \multirow{3}{*}{$8\times8$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN} \\
%        1\times1 \textrm{ conv, stride 2}
%      \end{bmatrix}\times 2$}  & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN} \\
%        1\times1 \textrm{ conv, stride 2}
%      \end{bmatrix}\times 2$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN}
%      \end{bmatrix}\times 2$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN} \\
%        1\times1 \textrm{ conv, stride 2}
%      \end{bmatrix}\times 2$}\\[0.5ex] 
%   & & & & &\\[0.5ex]
%   & & & & &\\[0.5ex]
% \hline
%   & & & & &\\[0.5ex]
% \multirow{3}{*}{Block (4)} & \multirow{3}{*}{$4\times4$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN} \\
%        1\times1 \textrm{ conv, stride 2}
%      \end{bmatrix}\times 2$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN} \\
%        1\times1 \textrm{ conv, stride 2}
%      \end{bmatrix}\times 2$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN} \\
%        1\times1 \textrm{ conv, stride 2}
%      \end{bmatrix}\times 2$} & \multirow{3}{*}{$\begin{bmatrix}
%        3\times3 \textrm{ conv, stride 2, BN, ReLU} \\
%        3\times3 \textrm{ conv, BN}
%      \end{bmatrix}\times 2$} \\[0.5ex] 
%   & & & & &\\[0.5ex]
%   & & & & &\\[0.5ex]
% \hline
% \makecell{Classification\\Layer}  & $1\times1$ & \multicolumn{4}{c}{$4\times4$ global average pool, 10D fully-connected, softmax} \\ [0.5ex]
% \hline

% \end{tabular}}
% \vspace{-1em}
% \label{table2}
% \end{table*}

% \subsection{Hybrid Architectures}
% \label{sec:ss_hybrid}
% The introduction of skip connections to the sequential style architecture has accelerated the performance of deep learning architectures. In past works, authors have focused on the effective length of the skip-connections. However, little thought has been given to the position of the skip-connections. For instance, in a 40-layer DenseNet with growth rate $k=12$ and reduction $r=1$, the last convolutional layer receives the input from all its previous layers aggregating to a 444 kernel input. We can always substitute these kernels by initializing the convolutional layer with the exact number of kernels. Now, one can easily argue whether it is the skip connection or the number of input kernels itself that is playing an important role. In order to test this we removed skip connections from layers in specific blocks, which represents the location of the skip-connection, and substituted them with an equivalent number of kernels. Consequently, this leads us to a "hybrid" style of architecture. The term hybrid basically represents a network which has a combination of skip and non-skip connections. One can extend the same argument to ResNets. 
% Furthermore, we removed skip-connection from each block of ResNets and DenseNets and evaluated the corresponding performance on both original testing and crafted adversarial images. A detailed configuration of the hybrid architectures are provided in Table \ref{table1}, \ref{table2}. Notably, removing skips from ResNets is easily understandable as the addition operator do not play with the number of input kernels to a layer.

% \begin{table*}[ht]
% \caption{Adversarial accuracy and smoothness score for different architectures tested on MNIST dataset
% }

% \centering
%  \begin{tabular}{c c c c c c}
% \hline
%   & & & & & \\
% \multirow{3}{*}{Models} & \multirow{3}{*}{Testing Acc.} & \multicolumn{2}{c}{Noise Level = 0.05} & \multicolumn{2}{c}{Noise Level = 0.1}\\[0.5ex]
%  &  & ------------- & ------------ & ------------- & ------------ \\ [0.5ex]
%  &  & Adv. Acc. & Score & Adv. Acc. & Score \\ [0.5ex]
% \hline
%  & & & & & \\
% MLP(3-layer\_100 neurons) & {97.39\%} & {59.37\%} & {0.26867} & {33.21\%} & {0.49371}\\ [0.5ex]
% MLP(3-layer\_200 neurons) & {97.87\%} & {71.38\%} & {0.18018} & {43.32\%} & {0.41408}\\ [0.5ex]
% LeNet & {99.23\%} & {79.75\%} & {0.13045} & {62.26\%} & {0.25883}\\ [0.5ex]\hline
%  \end{tabular} 
% \vspace{-1em}
% \label{table3}
% \end{table*}


% \begin{figure*}[ht]
% \caption{Adversarial accuracy and smoothness score for different architectures tested on MNIST dataset}
% \centering
% \scalebox{0.7}{
% \includegraphics[width=\textwidth]{mnist_chart.eps}
% }
% \label{figure2}
% \end{figure*}

% \begin{table*}[ht]
% \caption{Adversarial accuracy and smoothness score for different architectures tested on CIFAR-10 dataset
% }

% \centering
%  \begin{tabular}{c c c c c c}
%  \hline
%   & & & & & \\
% \multirow{3}{*}{Models} & \multirow{3}{*}{Testing Acc.} & \multicolumn{2}{c}{Noise Level = 0.3/255} & \multicolumn{2}{c}{Noise Level = 0.75/255}\\[0.5ex]
%  &  & ------------- & ------------ & ------------- & ------------ \\ [0.5ex]
%  &  & Adv. Acc. & Score & Adv. Acc. & Score \\ [0.5ex]
% \hline
%  & & & & & \\
% VGG16 & {94.38\%} & {81.55\%} & {0.07654} & {62.60\%} & {0.21269}\\ [0.5ex]
% ResNet18 & {95.49\%} & {81.40\%} & {0.08144} & {66.13\%} & {0.19240}\\ [0.5ex]
% ResNet18\_1block\_remove\_skip & {95.34\%} & {81.29\%} & {0.08296} & {66.51\%} & {0.19119}\\ [0.5ex]
% ResNet18\_2block\_remove\_skip & {95.26\%} & {80.56\%} & {0.08614} & {65.09\%} & {0.19793}\\ [0.5ex]
% ResNet18\_3block\_remove\_skip & {95.22\%} & {80.80\%} & {0.08643} & {63.59\%} & {0.21169}\\ [0.5ex]
% ResNet18\_4block\_remove\_skip & {95.37\%} & {82.53\%} & {0.07470} & {69.45\%} & {0.16911}\\ [0.5ex]
% DenseNet40\_12 & {94.82\%} & {72.31\%} & {0.13803} & {51.30\%} & {0.29069}\\ [0.5ex]
% DenseNet40\_12\_1block\_remove\_skip & {94.92\%} & {70.17\%} & {0.15588} & {50.33\%} & {0.30110}\\ [0.5ex]
% DenseNet40\_12\_2block\_remove\_skip & {94.45\%} & {76.73\%} & {0.10891} & {61.36\%} & {0.21918}\\ [0.5ex]
% DenseNet40\_12\_3block\_remove\_skip & {94.65\%} & {80.39\%} & {0.09189} & {71.72\%} & {0.15451}\\ [0.5ex]
%  \hline
%  \end{tabular} 
% \vspace{-1em}
% \label{table4}
% \end{table*}

% \begin{table*}[ht]
% \caption{Adversarial accuracy and smoothness score for different architectures tested on CIFAR-100 dataset
% }

% \centering
%  \begin{tabular}{c c c c c c}
%  \hline
%   & & & & & \\
% \multirow{3}{*}{Models} & \multirow{3}{*}{Testing Acc.} & \multicolumn{2}{c}{Noise Level = 0.3/255} & \multicolumn{2}{c}{Noise Level = 0.75/255}\\[0.5ex]
%  &  & ------------- & ------------ & ------------- & ------------ \\ [0.5ex]
%  &  & Adv. Acc. & Score & Adv. Acc. & Score \\ [0.5ex]
% \hline
%  & & & & & \\
% VGG16 & {73.95\%} & {52.35\%} & {0.11592} & {37.60\%} & {0.23297}\\ [0.5ex]
% ResNet18 & {78.76\%} & {52.74\%} & {0.10068} & {34.43\%} & {0.25286}\\ [0.5ex]
% ResNet18\_1block\_remove\_skip & {76.44\%} & {53.67\%} & {0.09212} & {34.44\%} & {0.25078}\\ [0.5ex]
% ResNet18\_2block\_remove\_skip & {76.36\%} & {52.97\%} & {0.09942} & {33.87\%} & {0.26117}\\ [0.5ex]
% ResNet18\_3block\_remove\_skip & {75.75\%} & {52.09\%} & {0.10099} & {35.03\%} & {0.24595}\\ [0.5ex]
% ResNet18\_4block\_remove\_skip & {76.19\%} & {52.96\%} & {0.09769} & {34.24\%} & {0.25655}\\ [0.5ex]
% DenseNet40\_12 & {72.24\%} & {36.60\%} & {0.18073} & {18.10\%} & {0.32471}\\ [0.5ex]
% DenseNet40\_12\_1block\_remove\_skip & {76.34\%} & {37.30\%} & {0.19169} & {20.52\%} & {0.32464}\\ [0.5ex]
% DenseNet40\_12\_2block\_remove\_skip & {77.38\%} & {44.30\%} & {0.17950} & {29.94\%} & {0.29787}\\ [0.5ex]
% DenseNet40\_12\_3block\_remove\_skip & {76.63\%} & {51.23\%} & {0.15466} & {42.30\%} & {0.22581}\\ [0.5ex]
%  \hline
%  \end{tabular} 
% \vspace{-1em}
% \label{table5}
% \end{table*}

% \begin{figure*}[ht]
% \caption{Adversarial accuracy and smoothness score for different architectures tested on CIFAR-100 dataset}
% \centering
% \includegraphics[width=\textwidth]{cifar100_chart.eps}
% \label{figure4}
% \end{figure*}



\subsection{Correlation analysis}
\label{sec:corr}
We observed that the proposed skewness score works transversely across cross-network frameworks. We found out that the skewness score, as compared to the adversarial accuracy at lower noise levels, was able to better predict the architectural performance at higher noises. This was verified by running some simple correlation tests between (skewness scores, adversarial error rate at $\epsilon=0.00293$ noise) and (adversarial accuracies at  $\epsilon = 0.3$, adversarial accuracies at $\epsilon=0.00293$ noise). In Table \ref{tab:correlation}, the first row of each cell illustrates the correlation analysis between the adversarial accuracies at $\epsilon = 0.00117$ with those at $\epsilon=0.00293$ noise. Second row details the correlation analysis for the skewness scores and adversarial error rate at $\epsilon=0.00293$ noise.
\begin{table}[ht]
\caption{Correlation tests for Skewness scores(SS) and Adversarial accuracies(AA) at lower noises ($\epsilon = 0.05$ for MNIST and $\epsilon = 0.00117$ for CIFAR and ImageNet) with accuracies for higher noises.
Each cell in the table illustrates the results for a particular dataset and attack.
}

\centering
 \begin{tabular}{c c c c c } %c c c c
 \hline
 & & & & \\ %& & 
\multirow{3}{*}{Datasets} & \multirow{3}{*}{Metric} & \multirow{3}{*}{Attack} & \multicolumn{2}{c}{Correlation statistics}\\[0.5ex] %& \multicolumn{2}{c}{$\epsilon= 0.00156$} & \multicolumn{2}{c}{$\epsilon= 0.00195$} 
 & &  & ------------- & ------------\\ [0.5ex] % & ------------- & ------------  & ------------- & ------------
 & &  & ${R}^2$ & p-value \\ [0.5ex] %${R}^2$ & p-value & ${R}^2$ & p-value & 
\hline
 & & & \\ %& & 
\multirow{2}{*}{MNIST} & AA & \multirow{2}{*}{GA} & \textbf{0.9358} & \textbf{0.1631}\\ [0.5ex] %{0.9876} & {6.53e-09} & {0.9559} & {1.06e-06} & 
& SS &  & {0.9017} & {0.2030}\\ [0.7ex] %{0.8557} & {0.0001} & {0.9033} & {2.485e-05} & 
\hline
\\
\multirow{2}{*}{MNIST} & AA & \multirow{2}{*}{GSA} & \textbf{0.9825} & \textbf{0.0844}\\ [0.5ex] %{0.9876} & {6.53e-09} & {0.9559} & {1.06e-06} & 
& SS &  & {0.9813} & {0.0874}\\ [0.7ex] %{0.8557} & {0.0001} & {0.9033} & {2.485e-05} & 
\hline
\\
\multirow{2}{*}{CIFAR-10} & AA &  \multirow{2}{*}{GA} & {0.8391} & {0.0005}\\ [0.5ex] %{0.9876} & {6.53e-09} & {0.9559} & {1.06e-06} & 
& SS &  & \textbf{0.9499} & \textbf{8.35e-06}\\ [0.7ex] %{0.8557} & {0.0001} & {0.9033} & {2.485e-05} & 
\hline
\\
\multirow{2}{*}{CIFAR-10} & AA &  \multirow{2}{*}{GSA} & {0.9160} & {5.16e-05}\\ [0.5ex] %{0.9920} & {1.14e-09} & {0.9781} & {6.33e-08} &
& SS &  & \textbf{0.9767} & \textbf{5.68e-07}\\ [0.7ex] %{0.9779} & {6.602e-08} & {0.9845} & {1.592e-08} & 
\hline
\\
\multirow{2}{*}{CIFAR-100} & AA &  \multirow{2}{*}{GA} & {0.7630} & {0.0021}\\ [0.5ex] %{0.9779} & {6.61e-08} & {0.9201} & {1.15e-05} & 
& SS &  & \textbf{0.8458} & \textbf{0.0004}\\ [0.7ex] %{0.4966} & {0.0228} & {0.6335} & {0.0059} & 
\hline
\\
\multirow{2}{*}{CIFAR-100} & AA &  \multirow{2}{*}{GSA} & {0.9071} & {0.1972}\\ [0.5ex] %{0.9898} & {3.02e-09} & {0.9683} & {2.79e-07} & 
& SS&  & \textbf{0.9586} & \textbf{0.1304}\\ [0.7ex] %{0.7412} & {0.0014} & {0.7950} & {0.0005} & 
\hline
\\
\multirow{2}{*}{ImageNet} & AA &  \multirow{2}{*}{GA} & {0.8879} & {0.0577}\\ [0.5ex] %{0.9917} & {0.0042} & {0.9662} & {0.0171} & 
& SS &  & \textbf{0.9431} & \textbf{0.0289}\\ [0.7ex] %{0.9924} & {0.0038} & {0.9884} & {0.0058} & 
\hline
\\
\multirow{2}{*}{ImageNet} & AA &  \multirow{2}{*}{GSA} & {0.8755} & {0.0643}\\ [0.5ex] % {0.9873} & {0.0064} & {0.9599} & {0.0202} &
& SS &  & \textbf{0.9304} & \textbf{0.0354}\\ [0.7ex] % {0.9946} & {0.0027} & {0.9849} & {0.0076} & 
 \hline
 \end{tabular} 
\vspace{-1em}
\label{tab:correlation}
\end{table}


%Surprisingly, a high performance contrast was found  between the skip-connected networks and their respective `hybrid' versions. We aim to get an understanding of the contribution of skip-connections at a particular location by constructing preliminary forms of hybrid architectures by removing skip-connections from all layers in specific blocks. For CIFAR-10, we discover that the skip-connections at the deeper stage contribute more to the adversarial performance. A keen observation is that hybrid networks do not affect the original validation accuracy of their parent architecture. Furthermore, for CIFAR-10 GA attack results, the adversarial performance increases by $\approx143\%$ for DenseNets and $\approx17\%$ for ResNets on increasing the perturbation from $\epsilon=0.00117$ to $0.00293$, when compared to their best hybrid versions respectively. For CIFAR-100 GA attack, adversarial performance increases by $\approx130\%$ for DenseNets and $\approx7\%$ for ResNets under the same noise settings. We observed a similar trend with respect to the other datasets and attacks. Notably, we see the error rates for the hybrid architectures were comparatively low across all architectures when compared to their primary counterparts.\\


% \begin{figure*}[t!]
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=95mm, height=75mm]{mnist_ga.eps}
%         \vspace{-3em}
%         \caption{Gradient Attack}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \includegraphics[width=95mm, height=75mm]{mnist_gsa.eps}
%         \vspace{-3em}
%         \caption{Gradient Sign Attack}
%     \end{subfigure}
%     \caption{Adversarial accuracy and Skewness score for different architectures tested on MNIST dataset for different attacks}
%     \label{fig:mnist}
% \end{figure*}

% \begin{figure*}[t!]
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=95mm, height=90mm]{cifar10_ga.eps}
%         \vspace{-5em}
%         \caption{Gradient Attack}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \includegraphics[width=95mm, height=90mm]{cifar10_gsa.eps}
%         \vspace{-5em}
%         \caption{Gradient Sign Attack}
%     \end{subfigure}
%     \vspace{-3.5em}
%     \caption{Adversarial accuracy and Skewness score for different architectures tested on CIFAR-10 dataset for different attacks}
%     \label{fig:cifar10}
% \end{figure*}

% \begin{figure*}[t!]
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=95mm, height=90mm]{cifar100_ga.eps}
%         \vspace{-5em}
%         \caption{Gradient Attack}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \includegraphics[width=95mm, height=90mm]{cifar100_gsa.eps}
%         \vspace{-5em}
%         \caption{Gradient Sign Attack}
%     \end{subfigure}
%     \vspace{-3.5em}
%     \caption{Adversarial accuracy and Skewness score for different architectures tested on CIFAR-100 dataset for different attacks}
%     \label{fig:cifar100}
% \end{figure*}

% \begin{figure*}[t!]
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=95mm, height=75mm]{imagenet_ga.eps}
%         \vspace{-3em}
%         \caption{Gradient Attack}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \includegraphics[width=95mm, height=75mm]{imagenet_gsa.eps}
%         \vspace{-3em}
%         \caption{Gradient Sign Attack}
%     \end{subfigure}
%     \caption{Adversarial accuracy and Skewness score for different architectures tested on ImageNet dataset for different attacks}
%     \label{fig:imagenet}
% \end{figure*}

% \begin{figure*}[ht]
% \centering
% \includegraphics[width=95mm, height=110mm]{cifar10_ga.eps}
% \vspace{-5.5em}
% \caption{Adversarial accuracy and Skewness score for different architectures tested on CIFAR-10 dataset for Gradient Attack}
% \label{fig:GAcifar10}
% \end{figure*}

% \begin{figure*}[ht]
% \centering
% \includegraphics[width=\textwidth, height=110mm]{cifar10_gsa.eps}
% \vspace{-5.5em}
% \caption{Adversarial accuracy and Skewness score for different architectures tested on CIFAR-10 dataset for Gradient Sign Attack}
% \label{fig:GSAcifar10}
% \end{figure*}

% \begin{figure*}[ht]
% \centering
% \includegraphics[width=\textwidth, height=110mm]{cifar100_ga.eps}
% \vspace{-5.5em}
% \caption{Adversarial accuracy and Skewness score for different architectures tested on CIFAR-100 dataset for Gradient Attack}
% \label{fig:GAcifar100}
% \end{figure*}

% \begin{figure*}[ht]
% \centering
% \includegraphics[width=\textwidth, height=110mm]{cifar100_gsa.eps}
% \vspace{-5.5em}
% \caption{Adversarial accuracy and Skewness score for different architectures tested on CIFAR-100 dataset for Gradient Sign Attack}
% \label{fig:GSAcifar100}
% \end{figure*}


% MNIST table
\begin{table*}[!h]
\caption{Adversarial accuracy and skewness score for different architectures tested on MNIST dataset
}
\centering
 \begin{tabular}{c c c c c c c c}
\hline
  & & & & & & &\\
  
Attack type & Models & Validation Acc. & \makecell{Adversarial Acc.\\ $\epsilon=0.05$} & \makecell{Adversarial Acc.\\ $\epsilon=0.1$} & 
\makecell{Adversarial Acc.\\ $\epsilon=0.15$} & \makecell{Adversarial Acc.\\ $\epsilon=0.2$} & Skewness score\\[0.5ex]
 &  &  &  &  &  &  &\\ [0.5ex]
\hline
 & & & & & \\
\multirow{3}{*}{FGM} & MLP1 & {97.39\%} & {59.37\%} & {33.21\%} & {28.86\%} & {27.94\%} & {2.4747}\\ [0.5ex]
& MLP2 & {97.87\%} & {71.38\%} & {43.22\%} & {38.29\%} & {36.65\%} & {1.9306}\\ [0.5ex]
& LeNet & {99.23\%} & {79.75\%} & {62.26\%} & {55.45\%} & {51.70\%} & {0.3923}\\ [0.5ex]
 &  &  &  &  &  &  &\\
\hline
 & & & & & \\
\multirow{3}{*}{FGSM} & MLP1 & {97.39\%} & {82.54\%} & {50.60\%} & {34.62\%} & {29.52\%} & {1.7377}\\ [0.5ex]
& MLP2 & {97.87\%} & {87.89\%} & {63.59\%} & {45.42\%} & {37.93\%} & {1.6304}\\ [0.5ex]
& LeNet & {99.23\%} & {94.38\%} & {79.40\%} & {66.34\%} & {54.59\%} & {0.2072}\\ [0.5ex]
\hline
 \end{tabular} 
\vspace{-1em}
\label{tab:MNIST}
\end{table*}

% CIFAR-10 table
\begin{table*}[!h]
\caption{Adversarial accuracy and skewness score for different architectures tested on CIFAR-10 dataset
}

\centering
 \begin{tabular}{c c c c c c c c}
\hline
  & & & & & & &\\
  
Attack type & Models & Validation Acc. & \makecell{Adversarial Acc.\\ $\epsilon=0.00117$} & \makecell{Adversarial Acc.\\ $\epsilon=0.00156$} & 
\makecell{Adversarial Acc.\\ $\epsilon=0.00195$} & \makecell{Adversarial Acc.\\ $\epsilon=0.00293$} & Skewness score\\[0.5ex]
 &  &  &  &  &  &  &\\ [0.5ex]
\hline
 & & & & & \\
\multirow{3}{*}{FGM} & DenseNet40 & {94.82\%} & {72.36\%} & {65.65\%} & {60.10\%} & {51.43\%} & {1.9316}\\ [0.5ex]
& ResNet18 & {95.49\%} & {81.48\%} & {77.40\%} & {73.28\%} & {66.17\%} & {0.8931}\\ [0.5ex]
& VGG13 & {94.10\%} & {81.76\%} & {76.97\%} & {72.78\%} & {63.55\%} & {0.9726}\\ [0.5ex]
 &  &  &  &  &  &  &\\
\hline
 & & & & & \\
\multirow{3}{*}{FGSM} & DenseNet40 & {94.82\%} & {80.07\%} & {74.03\%} & {68.25\%} & {56.54\%} & {1.6575}\\ [0.5ex]
& ResNet18 & {95.49\%} & {87.01\%} & {83.65\%} & {80.30\%} & {73.02\%} & {0.6567}\\ [0.5ex]
& VGG13 & {94.10\%} & {86.74\%} & {83.64\%} & {80.59\%} & {73.25\%} & {0.6558}\\ [0.5ex]
\hline
 \end{tabular} 
\vspace{-1em}
\label{tab:CIFAR10}
\end{table*}

% CIFAR-100 table
\begin{table*}[!h]
\caption{Adversarial accuracy and skewness score for different architectures tested on CIFAR-100 dataset
}

\centering
 \begin{tabular}{c c c c c c c c}
\hline
  & & & & & & &\\
  
Attack type & Models & Validation Acc. & \makecell{Adversarial Acc.\\ $\epsilon=0.00117$} & \makecell{Adversarial Acc.\\ $\epsilon=0.00156$} & 
\makecell{Adversarial Acc.\\ $\epsilon=0.00195$} & \makecell{Adversarial Acc.\\ $\epsilon=0.00293$} & Skewness score\\[0.5ex]
 &  &  &  &  &  &  &\\ [0.5ex]
\hline
 & & & & & \\
\multirow{3}{*}{FGM} & DenseNet40 & {75.78\%} & {41.82\%} & {34.79\%} & {29.65\%} & {21.12\%} & {3.2808}\\ [0.5ex]
& ResNet18 & {78.76\%} & {52.81\%} & {47.41\%} & {42.59\%} & {34.51\%} & {2.6733}\\ [0.5ex]
& VGG13 & {70.85\%} & {52.16\%} & {47.53\%} & {43.30\%} & {35.17\%} & {2.5241}\\ [0.5ex]
 &  &  &  &  &  &  &\\
\hline
 & & & & & \\
\multirow{3}{*}{FGSM} & DenseNet40 & {75.78\%} & {50.34\%} & {43.48\%} & {37.47\%} & {26.36\%} & {3.6574}\\ [0.5ex]
& ResNet18 & {78.76\%} & {59.18\%} & {53.91\%} & {49.25\%} & {39.80\%} & {2.7215}\\ [0.5ex]
& VGG13 & {70.85\%} & {57.68\%} & {53.56\%} & {49.92\%} & {42.38\%} & {2.2655}\\ [0.5ex]
\hline
 \end{tabular} 
\vspace{-1em}
\label{tab:CIFAR100}
\end{table*}

% IMAGENET table
\begin{table*}[h]
\caption{Adversarial accuracy and skewness score for different architectures tested on IMAGENET dataset
}

\centering
\begin{tabular}{c c c c c c c c}
\hline
  & & & & & & &\\
  
Attack type & Models & Validation Acc. & \makecell{Adversarial Acc.\\ $\epsilon=0.00117$} & \makecell{Adversarial Acc.\\ $\epsilon=0.00156$} & 
\makecell{Adversarial Acc.\\ $\epsilon=0.00195$} & \makecell{Adversarial Acc.\\ $\epsilon=0.00293$} & Skewness score\\[0.5ex]
 &  &  &  &  &  &  &\\ [0.5ex]
\hline
 & & & & & \\
\multirow{3}{*}{FGM} & VGG19\_bn & {74.22\%} & {13.17\%} & {9.58\%} & {7.69\%} & {5.65\%} & {1.2080}\\ [0.5ex]
& ResNet152 & {78.31\%} & {33.38\%} & {27.95\%} & {24.19\%} & {18.96\%} & {0.5638}\\ [0.5ex]
& DenseNet161 & {77.14\%} & {29.37\%} & {23.93\%} & {20.08\%} & {14.77\%} & {0.7149}\\ [0.5ex]
& InceptionV3 & {77.35\%} & {35.60\%} & {31.79\%} & {29.43\%} & {26.05\%} & {0.3091}\\ [0.5ex]
 &  &  &  &  &  &  &\\
\hline
 & & & & & \\
\multirow{3}{*}{FGSM} & VGG19\_bn & {74.22\%} & {20.74\%} & {14.58\%} & {10.82\%} & {6.48\%} & {1.2047}\\ [0.5ex]
& ResNet152 & {78.31\%} & {40.39\%} & {33.59\%} & {28.55\%} & {20.79\%} & {0.5428}\\ [0.5ex]
& DenseNet161 & {77.14\%} & {35.20\%} & {27.92\%} & {22.70\%} & {15.19\%} & {0.7055}\\ [0.5ex]
& InceptionV3 & {77.35\%} & {42.72\%} & {38.17\%} & {34.75\%} & {29.42\%} & {0.3371}\\ [0.5ex]
\hline
 \end{tabular} 
\vspace{-1em}
\label{tab:IMAGENET}
\end{table*}

